CELEUS: Certifiable and Efficient LLM Evaluation via E-Processes

Can we trust evaluation scores to capture an LLM's true real-world performance? Certifiable evaluation answers this question by providing a confidence interval (CI) that covers the LLM's true performance with high probability (e.g., 95%). In particular, existing methods sequentially select evaluation samples from a fixed pool and keep updating the CI until certain conditions are satisfied, e.g., the CI width reaches a target precision. However, existing methods are not generally anytime-valid: the claimed coverage (e.g., 95%) may fail when CIs are repeatedly updated and used to decide when to stop, leaving a gap between theoretical rigor and practice. This paper bridges this gap by proposing CELEUS, a Certifiable framework for Efficient LLM evaluation, which leverages E-processes to build anytime-valid CIs. Concretely, we propose a new signal that combines two ingredients: (i) Uncertainty-guided sampling to select informative samples for evaluation, and (ii) Surrogate-assisted approximations for unevaluated samples. We prove that the new signal remains unbiased for the evaluation score conditional on the past, enabling statistically-grounded and anytime-valid e-process CIs. More importantly, the two ingredients reduce estimation variance and help reach the target precision with fewer evaluated samples. We also prove that CIs obtained by CELEUS can shrink at a near-parametric rate up to logarithmic factors and analyze the oracle variance-optimal sampling rule that motivates the empirical uncertainty-guided one. Experiments show that CELEUS reaches the target precision using 54-62% fewer evaluated samples than baselines, while preserving anytime-valid coverage. Code is available at https://github.com/zyecs/celeus.

==> results/tab_rq2_labels_to_eps.tex <==
% \begin{table}[t]
% \centering
% \small
% \caption{Median labels needed to reach precision $\epsilon=0.05$, pooled by dataset (median across the four pairs of Tab.~(\ref{tab:setup-pairs})). No method failed to reach $\epsilon$ within $t_{\max}$ on any cell. \bo{bold the winner or in this case, you can add like ``- xxx" to CELEUS column to emphasize its improvements}}
% \label{tab:rq2-labels-to-eps}
% \begin{tabular}{lcccccc}
% \toprule
% Dataset & \ourmethod & \evbaseline & \cereval & Oracle & Rel. savings \\
% \midrule
% \textsc{SST-2}   & $3{,}835$ & $13{,}886$ & \zs{[pending]} & $2{,}822$ & $72.4\%$ \\
% \textsc{MMLU}    & $3{,}692$ & $9{,}654$  & \zs{[pending]} & $2{,}395$ & $61.8\%$ \\
% \textsc{AG News} & $6{,}598$ & $15{,}384$ & \zs{[pending]} & $4{,}325$ & $57.1\%$ \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{minipage}{0.6\linewidth}
% \centering
% \small
% \caption{Median number of used labels to reach $\epsilon=0.05$ on each benchmark, across the four surrogate-target pairs and $50$ independent runs.
% No method fails to reach $\epsilon$ within $t_{\max}$.
% We mark the relative savings of \ourmethod~vs.\ \evbaseline, and the \textbf{top-performer} in bold.
% \oracleacq\ is included for reference only.
% }
% \label{tab:labels-to-eps}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccc}
% \toprule
%                        & SST-2 & MMLU & AG\,News \\
%                        & {\scriptsize ($N{=}68{,}221$)} & {\scriptsize ($N{=}115{,}700$)} & {\scriptsize ($N{=}127{,}600$)} \\
% \midrule
% \evbaseline            & $5{,}723$                                  & $6{,}524$                                  & $14{,}914$                                 \\
% \nosurr                & $5{,}517_{\text{\,($-4\%$)}}$              & $3{,}940_{\text{\,($-40\%$)}}$             & $7{,}692_{\text{\,($-48\%$)}}$             \\
% \ourmethod    & $\mathbf{2{,}936_{\text{\,($-49\%$)}}}$    & $\mathbf{2{,}592_{\text{\,($-60\%$)}}}$    & $\mathbf{7{,}103_{\text{\,($-52\%$)}}}$    \\
% \midrule
% % \rowcolor{lightgray}
% % \textit{\oracleacq} & \textit{$2{,}526$} & \textit{$1{,}661$} & \textit{$3{,}917$} \\
% {\color{gray}\oracleacq} & {\color{gray}$2{,}526$} & {\color{gray}$1{,}661$} & {\color{gray}$3{,}917$} \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}
% \end{table}

==> results/tab_setup_pairs.tex <==
\begin{table}[t]
\centering
\small
\caption{Surrogate-target pairs used throughout our experiments. 
Higher $\rho$ (i.e., Spearman correlation, computed over seeds and datasets) indicates a more informative surrogate; the column serves as the empirical axis along which later figures should be read. 
Family match is "Y" iff the surrogate and target belong to the same training family. 
Mixtral parameter count is reported as active parameters per token.}
\label{tab:setup-pairs}
\begin{tabular}{llccc}
\toprule
Surrogate & Target & Family match & Size gap & $\rho$ \\
\midrule
\textsc{Llama2-7B}  & \textsc{Mixtral-8$\times$7B} & N & 7B$\rightarrow$46B & $0.48$ \\
\textsc{Llama2-7B}  & \textsc{Llama3-70B}          & N & 7B$\rightarrow$70B & $0.45$ \\
\textsc{Llama3-8B}  & \textsc{DeepSeek-67B}        & N & 8B$\rightarrow$67B & $0.43$ \\
\textsc{Llama3-8B}  & \textsc{Llama3-70B}          & Y & 8B$\rightarrow$70B & $0.41$ \\
\bottomrule
\end{tabular}
\end{table}
